A Dense Reward View on Aligning Text-to-Image Diffusion with Preference

Aligning text-to-image diffusion model (T2I) with preference has been gaining increasing research attention. While prior works exist on directly optimizing T2I by preference data, these methods are developed under the bandit assumption of a latent reward on the entire diffusion reverse chain, while ignoring the sequential nature of the generation process. This may harm the efficacy and efficiency of preference alignment. In this paper, we take on a finer dense reward perspective and derive a tractable alignment objective that emphasizes the initial steps of the T2I reverse chain. In particular, we introduce temporal discounting into DPO-style explicit-reward-free objectives, to break the temporal symmetry therein and suit the T2I generation hierarchy. In experiments on single and multiple prompt generation, our method is competitive with strong relevant baselines, both quantitatively and qualitatively. Further investigations are conducted to illustrate the insight of our approach.

==> Tex/background.tex <==
\section{Background} \label{sec:background}

==> Tex/tab/clip_score_single_prompt.tex <==
\begin{table}[H]
\captionsetup{font=small}
\caption{
\small
CLIP scores for the single-prompt experiment in \cref{sec:exp_single}, where seen and unseen prompts are tabulated in \cref{table:four_single_prompts}.
Shown are the scores of our method and the baselines in \cref{fig:single_prompt_generated_images}.
``Traj.'' denotes the classical DPO-style objective discussed in \Secref{sec:connect_with_dpo}, \ie, assuming trajectory-level reward. 
Best score in each prompt is bold.
It is clear that our method improves image-text matching.
} 
\label{table:clip_score_single_prompt}
\centering 
% \vspace{-.5em}
% \setlength\tabcolsep{12pt}
% \renewcommand{\arraystretch}{1.1}
% \resizebox{1.\textwidth}{!}
% {
% \footnotesize
\begin{tabular}{@{}lccccccccc@{}}
\toprule
                        & \multicolumn{4}{c}{Seen Prompt}                                   &  & \multicolumn{4}{c}{Unseen Prompt}                                 \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
                        & Color          & Count          & Composition    & Location       &  & Color          & Count          & Composition    & Location       \\ \midrule
SD1.5                   & 34.50          & 34.20          & 28.45          & 32.56          &  & 36.00          & 36.22          & 36.74          & 36.52          \\
DPOK                    & 37.19          & 34.91          & 31.33          & 37.02          &  & 37.08          & 38.51          & 36.87          & 38.00          \\
Traj. & 37.44          & 35.36          & 30.90          & 37.88          &  & 36.65          & 38.62          & 36.92          & 38.43          \\
Ours                    & \textbf{37.91} & \textbf{35.81} & \textbf{32.20} & \textbf{38.35} &  & \textbf{37.54} & \textbf{39.18} & \textbf{37.44} & \textbf{39.90} \\ \bottomrule
\end{tabular}
% }
\end{table}
